MegaVul: A C/C++ Vulnerability Dataset with Comprehensive Code Representation

We constructed a newly large-scale and comprehensive C/C++ vulnerability dataset named MegaVul by crawling the Common Vulnerabilities and Exposures (CVE) database and CVE-related open-source projects. Specifically, we collected all crawlable descriptive information of the vulnerabilities from the CVE database and extracted all vulnerability-related code changes from 28 Git-based websites. We adopt advanced tools to ensure the extracted code integrality and enrich the code with four different transformed representations. In total, MegaVul contains 17,380 vulnerabilities collected from 992 open-source repositories spanning 169 different vulnerability types disclosed from January 2006 to October 2023. Thus, MegaVul can be used for a variety of software security-related tasks including detecting vulnerabilities and assessing vulnerability severity. All information is stored in the JSON format for easy usage. MegaVul is publicly available on GitHub and will be continuously updated. It can be easily extended to other programming languages.

==> sections/dataset-backup.tex <==
\subsection{Dataset Construction---backup}

% \chao{introduction to our extended dataset, which should include what are the new contributions of our dataset and how we build such a dataset }


    


{
\textbf{Data Source} The National Vulnerability Database(NVD)\cite{nvd} is a public resource maintained by NIST to collect, organize and distribute information on security vulnerabilities in software products, which is a good starting-point for collecting a high-quality, comprehensive dataset for vulnerability detection. We scraped the all available Common Vulnerabilities and Exposures(CVE)\cite{cve} entries from the dataset in JSON format provided by the NVD.
By collecting these CVE entries, we can extract valuable descriptive information such as the CVE IDs, CVE summary, CVSS severity scores, and reference links to relevant products or patches for fixing the vulnerabilities.
Then we dug into the vulnerability fix commits for each CVE.
For each vulnerability fix commit, we follow Chakraborty et al.'s\cite{chakraborty2021deep} approach of annotating previous version of modified functions in the commit (i.e. the parent commit) as vulnerable, while considering the current version of the modified function as non-vulnerable. 
Moreover, those functions that remain unchanged are annotated as non-vulnerable.
In summary we need to download metadata and modified files for the vulnerability fix commit, and the corresponding parent commit.
Through manual analysis of the referenced commit links in CVE entries, we identified 17 Git code hosting platform from 349 websites that had referenced the CVE entries more than 100 times. 
The web-based code hosting platforms can be categorized into five main categories: Github, GitLab, GitWeb, CGit, and Gitiles.
We implement logic to download commits for each platform individually, while also ensuring the integrity of the downloaded commit. For example, we utilize the official GitHub API to handle downloads from GitHub, and employ crawler for GitWeb to traverse the commit's metadata and extract the download path of the files.
Ultimately, we successfully obtained 8,334 commits from 198994 CVE entries through the download process.
}

{
\textbf{Function Extract}
Our dataset aims to collect function-level vulnerabilities in C/C++ code, which constitute the vast majority of vulnerabilities recorded in the NVD database.
For files included in the commit, we gather C/C++ related source code and headers based on their file extensions, while filtering out any other files.
In the next step, we need to separate the functions in the file. 
Existing datasets are implemented through predefined rules or by using regular expression tools like lizard. However, these methods have limitations due to their simplicity. 
For example, regular expressions cannot fully represent the complex syntax rules of the C-like language. 
As a result, these methods may result in the extraction of incomplete functions or the incorrect separation of multiple functions into a single function.
We used the syntax rule-based parser tree-sitter to separate functions, and on top of that extended the syntax rules to identify more macro modifiers frequently used by popular open source projects, such as the macro modifier \textit{\_\_init} defined in Linux.
Furthermore, we temporarily remove the macros from the code before parsing, which allows the parser to effectively and accurately separate the functions without the interference of macros.
% We ended up with \textcolor{red}{xxx} previous and current version of the function from \textcolor{red}{xxx} commits with code changes. 
% Furthermore, we additionally extract \textcolor{red}{xxx} functions that remained unchanged between the previous and current version of the commits.
}

{
\textbf{Post-processing}
At this stage, we perform filtering on the dataset and enrich the information within it. 
Specifically, we employ three filtering strategies to further enhance the quality of the data:
1) Filtering functions with more than 5,000 lines of code. Most of these functions are automatically generated by lexer parsers such as Antlr and Yacc.
2) Removing newly added functions in commits. This is because we cannot determine whether they contain vulnerabilities.
3) Filtering functions with more than 1,000 lines of code changes. These functions may involve code refactoring. To avoid excessive complexity and maintain the significance of subsequent analysis, we have filtered out large-scale code changes.
Existing datasets solely provide the string representation of functions, disregarding other dimensional information of functions that numerous deep learning-based vulnerability detection models rely on. For example, 
Graph-based\cite{chakraborty2021deep,zhou2019devign,li2021vulnerability} models leverage function's AST, CPG\cite{cpg-yamaguchi2014modeling}, and other graph structures to effectively capture the syntactic and semantic characteristics of code. Token-based sequence models address the problem of vocabulary explosion by abstracting specific elements, such as substituting variable names with symbolic names like "VAR" \cite{li2021sysevr}. Vul4C, in contrast, addresses these limitations by offering more comprehensive dimensional information. 
Not only does this approach liberate researchers from the repetitive task of implementing the necessary logic, but by incorporating a fixed version of the data, it facilitates a fair comparison and evaluation of various vulnerability detection models.
Consequently, Vul4C provides information on the four dimensions of the function, which include: 
1) Function signature: This includes the function name, a comprehensive list of arguments with their respective names and types, and the return type of the function.
2) Abstracted function: Nine levels of granularity abstraction (e.g. FUNC, VAR, STRING) and corresponding mappings.
3) Parsed Function by Joern: The \textit{Joern}\cite{joern} tool statically parses functions, generating graph representations that offer insights into their structure and dependencies. These representations include Abstract Syntax Trees (AST), Program Dependence Graphs (PDG)\cite{cpg-ferrante1987program}, and more.
4) Code changes: Details of function changes are generated using the \textit{diff}\cite{git} tool, including line level modifications, additions and deletions.}

{
The Vul4C dataset initially collected 8,234 raw commits based on the CVE entries recorded in the NVD dataset. After the Function Extract and Post-processing phases, we ended up with 6,437 commits covering 736 different projects. In total, from the 8,795 modified files, we extracted approximately 14,000 vulnerable functions across 159 CWE types, as well as 377,000 functions without vulnerabilities.
We distribute Vul4C and its build scripts for future research.
}

\begin{table}[htbp]
  \centering
  \caption{Descriptive statistics for \datasetname and BigVul}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|r|r}
    \toprule
 & Vul4C & BigVul\\
\midrule

Number of Projects & 736 & 310\\
Number of CVE IDs & 5714 & 3539\\
Date range of crawled CVEs & 2013/01-2023/04 & 2013/01-2019/03 \\
Number of CWE IDs & 159 & 92\\
Number of Commits & 6437 & 4058\\
\makecell{Number of \\ Crawled Code Hosting Platform }  &  17 & 2 \\
Number of Vul/Non-Vul Function & 14216/377185 & 10900/177736  \\ 
Function Extract Strategy/(Quality)  & Tree-sitter(High) &  Lizard(Low) \\ 
Dimensions of Information & 
% \makecell{CVSS,Diff info, Commit structure \\ \textit{Nine-granularity} abstraction \\ \textit{Joern} graph,function signature}
% & CVSS,Diff info \\
6 & 2 \\
Code Availability & Full & Partial \\
\bottomrule
\end{tabular}}
\label{tab:vul4c}
\end{table}


